Ultrafast Grid Impedance Identification in $dq$-Asymmetric Three-Phase Power Systems

We propose a non-parametric frequency-domain method to identify small-signal $dq$-asymmetric grid impedances, over a wide frequency band, using grid-connected converters. Existing identification methods are faced with significant trade-offs: e.g., passive approaches rely on ambient harmonics and rare grid events and thus can only provide estimates at a few frequencies, while many active approaches that intentionally perturb grid operation require long time series measurement and specialized equipment. Although active time-domain methods reduce the measurement time, they either make crude simplifying assumptions or require laborious model order tuning. Our approach effectively addresses these challenges: it does not require specialized excitation signals or hardware and achieves ultrafast ($<1$ s) identification, drastically reducing measurement time. Being non-parametric, our approach also makes no assumptions on the grid structure. A detailed electromagnetic transient simulation is used to validate the method and demonstrate its clear superiority over existing alternatives.

==> config/macros.tex <==
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother


\newcommand{\mo}[1]{{\color{cyan} \smallskip\emph{Mohamed}: #1\smallskip}}

\providecommand{\eu}{\ensuremath{\mathrm{e}}}

\makeatletter
\providecommand*{\diff}%
{\@ifnextchar^{\DIfF}{\DIfF^{}}}
\def\DIfF^#1{%
\mathop{\mathrm{\mathstrut d}}%
\nolimits^{#1}\gobblespace}
\def\gobblespace{%
\futurelet\diffarg\opspace}
\def\opspace{%
\let\DiffSpace\!%
\ifx\diffarg(%
\let\DiffSpace\relax
\else
\ifx\diffarg[%
\let\DiffSpace\relax
\else
\ifx\diffarg\{%
\let\DiffSpace\relax
\fi\fi\fi\DiffSpace}


\providecommand*{\deriv}[3][]{%
\frac{\diff^{#1}#2}{\diff #3^{#1}}}

\newcommand{\vc}{\mathrm{vec}}
\newcommand{\paren}[1]{\ensuremath{\left( #1\right)}}
\newcommand{\sparen}[1]{\ensuremath{(#1)}}
\newcommand{\clint}[1]{\ensuremath{\left[ #1\right]}}
\newcommand{\set}[1]{\ensuremath{\left\{ #1\right\}}}
\newcommand{\matr}[1]{\ensuremath{\begin{bmatrix} #1 \end{bmatrix}}}
\newcommand{\norm}[1]{\ensuremath{\left\| #1\right\|}}
\newcommand{\snorm}[1]{\ensuremath{\| #1\|}}
\newcommand{\abs}[1]{\ensuremath{\left| #1\right|}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\opnorm}[1]{\ensuremath{\| #1\|_{\mathrm{op}}}}
\newcommand{\hsnorm}[1]{\ensuremath{\| #1\|_{\mathrm{F}}}}
\newcommand{\hinfnorm}[1]{\ensuremath{\| #1\|_{\mathcal{H}_{\infty}}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\toep}{\mathcal{T}}
\newcommand{\cconv}{\circledast}
\newcommand{\conv}{*}
\renewcommand{\Pr}{\mathbb{P}}

\newcommand{\du}{d_{{u}}}
\newcommand{\Du}{D_{{u}}}
\newcommand{\cu}{c_{{u}}}
\newcommand{\sigmau}{\sigma_{{u}}}
\newcommand{\sigmae}{\sigma_{{e}}}
\newcommand{\dy}{d_{{y}}}
\newcommand{\de}{d_{{e}}}
\newcommand{\Np}{N_p}
\newcommand{\Ntot}{N_\mathrm{tot}}
\newcommand{\cplx}{\mathbb{C}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\blkdiag}{\mathrm{blkdiag}}
\newcommand{\p}{\mathrm{\mathstrut p}}
\newcommand{\A}{\mathcal{A}}


\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bE}{\boldsymbol{E}}

\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\1}{\boldsymbol{1}}


\newcommand{\F}{\mathcal{F}}



% for the square hat used in the Appendix
% requires the package: stackengine
\def\rlwd{.4pt}
\def\rlht{1.1pt}
\def\shatvrule{\rule{\rlwd}{\rlht}}
\def\shat#1{%
  \setbox0=\hbox{$#1$}%
  \stackon[0pt]{\stackon[1pt]{\ensuremath{#1}}{%
    \shatvrule\kern\wd0\kern-\rlwd\kern-\rlwd\shatvrule}}%
    {\rule{\wd0}{\rlwd}}%
}
